The Importance of Autonomous Driving Using 5G Technology

The three keys to autonomous driving are sensors, data integration, and 100% safety decisions. In the past, due to the high latency and low reliability of the network, many decisions had to be made locally in the vehicle. This puts high demands on the vehicle itself, which results in the dilatory commercialization of automatic driving. With the advent of 5G, these situations will be greatly improved. In this paper, we present the improvements that 5G technology brings to autonomous vehicles especially in terms of latency and reliability amongst the multitude of other factors. The paper analyzes the specific areas where 5G can improve for autonomous vehicles and Intelligent Transport Systems in general (ITS) and looks forward to the application of 5G technology in the future.

==> 6_future.tex <==
\section{Discussion and Future Work}
Future autonomous driving will be combined with edge computing. Autonomous driving is indeed just the beginning on the road to commercialization. With 5G driving, autonomous driving will be a promising prospect in the future. The 5G communication will also be divided amongst various industries like entertainment, consumer usage, technology industries and so it is also of utmost importance to see how and what proportion of the network is dedicated to autonomous vehicles. Various papers suggest different slicing of the network to utilize it at full efficiency. \cite{8246845}

Through 5G remote control, under the "boundary conditions" that autonomous driving has not learned, it can freely switch to human remote control mode, more accurately handle complex driving scenarios. It will greatly reduce the cost of research and development of autonomous driving technology. At the same time, 5G remote assistance will also improve the operational dispatching efficiency of large-scale autonomous driving fleets. In the future, remote customer service can also be added to meet passenger demands in real-time.

The car of the future is not only a means of transportation but also the development of a new generation of Internet terminals, enabling the car to separate from the driver and ensure driving maneuverability and safety. Autonomous driving fundamentally changes the control mode of traditional cars, which has a greater guarantee for the safety and efficiency of traffic systems.

The other important part that 5G would affect autonomous vehicles is in the law. In other words, 5G will also promote the development of regulatory standards. There are still many industry standards for the development of the autonomous driving industry. Different car companies, whether traditional car companies or new car companies are exploring. It is foreseeable that with the addition of 5G technology, the autonomous driving industry will have a period of accelerated development in a short period. Besides, there is also a very important topic, which is the introduction and improvement of related industry standards, laws and regulations. 
